Hybrid performance modelling of opportunistic networks

We demonstrate the modelling of opportunistic networks using the process algebra stochastic HYPE. Network traffic is modelled as continuous flows, contact between nodes in the network is modelled stochastically, and instantaneous decisions are modelled as discrete events. Our model describes a network of stationary video sensors with a mobile ferry which collects data from the sensors and delivers it to the base station. We consider different mobility models and different buffer sizes for the ferries. This case study illustrates the flexibility and expressive power of stochastic HYPE. We also discuss the software that enables us to describe stochastic HYPE models and simulate them.

==> eptcsdata.tex <==
\providecommand{\firstpage}{106}
\providecommand{\publicationstatus}{M. Massink and H. Wiklicky (Eds.):Workshop on Quantitative\\
Aspects of Programming Languages and Systems 2012 (QAPL 2012)\\
EPTCS 85, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.85.8}{10.4204/EPTCS.85.8}}
\pdfoutput=1

